A Semantic Model for Interacting Cyber-Physical Systems

We propose a component-based semantic model for Cyber-Physical Systems (CPSs) wherein the notion of a component abstracts the internal details of both cyber and physical processes, to expose a uniform semantic model of their externally observable behaviors expressed as sets of sequences of observations. We introduce algebraic operations on such sequences to model different kinds of component composition. These composition operators yield the externally observable behavior of their resulting composite components through specifications of interactions of the behaviors of their constituent components, as they, e.g., synchronize with or mutually exclude each other's alternative behaviors. Our framework is expressive enough to allow articulation of properties that coordinate desired interactions among composed components within the framework, also as component behavior. We demonstrate the usefulness of our formalism through examples of coordination properties in a CPS consisting of two robots interacting through shared physical resources.

==> eptcsdata.tex <==
\providecommand{\firstpage}{77}
\providecommand{\publicationstatus}{J. Lange, A. Mavridou, L. Safina, A. Scalas (Eds.):\\
14th Interaction and Concurrency Experience (ICE 2021).\\
EPTCS 347, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.347.5}{10.4204/EPTCS.347.5}}

